New Directions in Automated Traffic Analysis

Despite the use of machine learning for many network traffic analysis tasks in security, from application identification to intrusion detection, the aspects of the machine learning pipeline that ultimately determine the performance of the model -- feature selection and representation, model selection, and parameter tuning -- remain manual and painstaking. This paper presents a method to automate many aspects of traffic analysis, making it easier to apply machine learning techniques to a wider variety of traffic analysis tasks. We introduce nPrint, a tool that generates a unified packet representation that is amenable for representation learning and model training. We integrate nPrint with automated machine learning (AutoML), resulting in nPrintML, a public system that largely eliminates feature extraction and model tuning for a wide variety of traffic analysis tasks. We have evaluated nPrintML on eight separate traffic analysis tasks and released nPrint and nPrintML to enable future work to extend these methods.

==> figures/active/dataset.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
    \centering
    \small
\begin{tabular}{@{}lcr@{}}
\toprule
Vendor     & Device Type    & Labeled Devices \\ \midrule
Adtran     & Network Device & 1,449              \\
\rowcolor{Gray}
Avtech     & IoT Camera     & 2,152              \\
Axis       & IoT Camera     & 2,653              \\
\rowcolor{Gray}
Chromecast & IoT Streaming  & 2,872              \\
Cisco      & Network Device & 1,451              \\
\rowcolor{Gray}
Dell       & Network Device & 1,449              \\
H3C        & Network Device & 1,380              \\
\rowcolor{Gray}
Huawei     & Network Device & 1,409              \\
Juniper    & Network Device & 1,445              \\ 
\rowcolor{Gray}
Lancom     & Network Device & 1,426              \\
Miktrotik  & Network Device & 1,358              \\ 
\rowcolor{Gray}
NEC        & Network Device & 1,450              \\
Roku       & IoT Streaming  & 2,403              \\ 
\rowcolor{Gray}
Ubiquoss   & Network Device & 1,476              \\
ZTE        & Network Device & 1,425              \\ \bottomrule
\end{tabular}
    \caption{The active device fingerprinting dataset.}
    \label{tab:active-dataset}
\end{table}


==> figures/active/nmap-eval.tex <==
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
    \centering
    \small
    % \resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lrrr@{}}
\toprule
\multicolumn{1}{c}{Representation} &
    \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Balanced\\
    Accuracy\end{tabular}} & \multicolumn{1}{c}{ROC AUC}  &
    \multicolumn{1}{c}{F1} \\ \midrule
nPrint                             & 95.4  & 99.7                         & 95.5                         \\
    \rowcolor{Gray} Nmap       & 92.7                                                    & 99.3 &    92.9 \\ \bottomrule
\end{tabular}
    % } %
    \caption{Models trained on the \name{} representation outperform Nmap's
    hand-engineered features across every metric considered.}
    \label{tab:nmap-perf}
\end{table}


==> figures/active/nmap-heuristic.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
    \centering
 \resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lcrrrrr@{}}
\toprule
           & \multicolumn{1}{l}{}                                   & \multicolumn{1}{l}{}                                                           & \multicolumn{2}{c}{Nmap Direct}                            & \multicolumn{2}{c}{Nmap Aggressive}                        \\ \cmidrule(l){4-7} 
Vendor     & \begin{tabular}[c]{@{}c@{}}Device \\ Type\end{tabular} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Labeled \\ Devices\end{tabular}} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall} \\ \midrule
Adtran     & Network                                                & 1,449                                                                          & 0.95                          & 0.24                       & 0.70                          & 1.00                       \\
    \rowcolor{Gray} Avtech     & IoT                                                    & 2,152                                                                          & 0.00                          & 0.00                       & 0.00                          & 0.03                       \\
Axis       & IoT                                                    & 2,653                                                                          & 0.00                          & 0.00                       & 0.01                          & 0.52                       \\
    \rowcolor{Gray} Chromecast & IoT                                                    & 2,872                                                                          & 0.00                          & 0.00                       & 0.00                          & 0.33                       \\
Cisco      & Network                                                & 1,451                                                                          & 0.99                          & 0.56                       & 0.95                          & 0.99                       \\
 \rowcolor{Gray} Dell       & Network                                                & 1,449                                                                          & 0.11                          & 0.27                       & 0.11                          & 0.87                       \\
H3C        & Network                                                & 1,380                                                                          & 0.00                          & 0.00                       & 0.31                          & 0.85                       \\
 \rowcolor{Gray} Huawei     & Network                                                & 1,409                                                                          & 0.76                          & 0.24                       & 0.55                          & 0.87                       \\
Juniper    & Network                                                & 1,445                                                                          & 0.99                          & 0.48                       & 0.72                          & 0.98                       \\
 \rowcolor{Gray} Lancom     & Network                                                & 1,426                                                                          & 0.05                          & 0.00                       & 0.15                          & 0.84                       \\
Mikrotik   & Network                                                & 1,358                                                                          & 0.00                          & 0.00                       & 0.04                          & 0.47                       \\
 \rowcolor{Gray} NEC        & Network                                                & 1,450                                                                          & 0.00                          & 0.00                       & 0.60                          & 0.99                       \\
Roku       & IoT                                                    & 2,403                                                                          & 0.00                          & 0.00                       & 0.00                          & 0.00                       \\
 \rowcolor{Gray} Ubiquoss   & Network                                                & 1,476                                                                          & 0.00                          & 0.00                       & 0.00                          & 0.00                       \\
ZTE        & Network                                                & 1,425                                                                          & 0.00                          & 0.00                       & 0.00                          & 0.00                       \\ \bottomrule
\end{tabular}
    }%
    \caption{The active device fingerprinting set and Nmap's heuristic
    performance on the devices. Nmap's heuristic only excels on Cisco devices, with
    significantly lower performance across IoT devices.}
    \label{tab:nmap-heuristic}
\end{table}


==> figures/active/nprint-vs-nmap.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
    \small
    \centering
\begin{tabular}{@{}lcc@{}}
\toprule
                           & \multicolumn{2}{c}{Average Precision}                                                                       \\ \cmidrule(l){2-3} 
\multicolumn{1}{l}{Vendor} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}ML-Enhanced\\ Nmap\end{tabular}} & \multicolumn{1}{c}{nPrint} \\ \midrule
Adtran                     & 1.00                                                                           & 1.00                       \\
\rowcolor{Gray} 
Avtech                     & 0.87                                                                           & 0.95                       \\
Axis                       & 0.93                                                                           & 0.98                       \\
\rowcolor{Gray} 
Chromecast                 & 1.00                                                                           & 1.00                       \\
Cisco                      & 0.97                                                                           & 0.99                       \\
\rowcolor{Gray} 
Dell                       & 0.85                                                                           & 0.99                       \\
H3C                        & 0.95                                                                           & 0.96                       \\
\rowcolor{Gray} 
Huawei                     & 0.94                                                                           & 0.95                       \\
Juniper                    & 0.99                                                                           & 0.99                       \\
\rowcolor{Gray} 
Lancom                     & 0.99                                                                           & 0.99                       \\
Mikrotik                   & 0.88                                                                           & 0.91                       \\
\rowcolor{Gray} 
NEC                        & 1.00                                                                           & 1.00                       \\
Roku                       & 0.92                                                                           & 0.99                       \\
\rowcolor{Gray} 
Ubiquoss                   & 0.99                                                                           & 0.99                       \\
ZTE                        & 0.99                                                                           & 0.99                       \\ \bottomrule
\end{tabular}
    \caption{Models trained on the \name{} representation match or outperform models trained on Nmap's hand-engineered features for every class in the dataset.}
    \label{tab:nprintvsnmap}

\end{table}


==> figures/active/time.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
    \centering
    \small
     \resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lrrrr@{}}
\toprule
\multicolumn{1}{c}{Representation} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\# Models in\\ Ensemble\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Training Time\\ (Seconds)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Inference Time\\ (Seconds)\end{tabular}} & \multicolumn{1}{c}{F1} \\ \midrule
Nmap                               & 2                                                                                   & 497                                                                                   & 12                                                                                     & 92.8                   \\
\rowcolor{Gray} 
Nmap                               & 3                                                                                   & 630                                                                                   & 32                                                                                     & 92.9                   \\
nPrint                             & 3                                                                                   & 755                                                                                   & 267                                                                                    & 95.4                   \\
\rowcolor{Gray} 
nPrint                             & 2                                                                                   & 188                                                                                   & 3                                                                                      & 95.2                   \\ \bottomrule
\end{tabular}
    }
    \caption{Ensembles of models trained on the \name{} representation can outperform Nmap in both F1 score
    and inference time.}
    \label{tab:active-time}
\end{table}


==> figures/app/dataset.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs} \usepackage[table,xcdraw]{xcolor} If you use beamer only
% pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{table}[t]
\centering
\small
    % \resizebox{\columnwidth}{!}{%
\begin{tabular}{lrrrr}
    \toprule
        & \multicolumn{4}{c}{Application Handshakes} \\ \cmidrule{2-5} 
Browser & Snowflake  & Facebook  & Google  & Discord \\ \midrule
Firefox & 991        & 796       & 1000    & 992     \\
\rowcolor{Gray}
Chrome  & 0          & 784       & 995     & 997     \\ \bottomrule
\end{tabular}
    % }%
    \caption{The application identification dataset~\cite{macmillan2020evaluating}.}
    \label{tab:app-dataset}
\end{table}


==> figures/app/perf.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs} \usepackage[table,xcdraw]{xcolor} If you use beamer only
% pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
    \centering
    \normalsize
    \begin{tabular}{@{}lrrr@{}}
        \toprule
        Model & Accuracy & ROC AUC & F1   \\ \midrule FFN   & 99.8         &  99.8
              & 99.8                      \\
        \rowcolor{Gray}
        CNN   & 100.0    & 100.0    & 100.0 \\
        RF    & 99.4     & 100.0    & 99.4 \\ \bottomrule
    \end{tabular}
    \caption{Performance of models trained on the \name{} representation. We see high performance
        in each model, with the CNN achieving perfect performance in all metrics
        considered.}
    \label{tab:app-perf}
\end{table}


==> figures/app/time.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
    \centering
    \small
\begin{tabular}{@{}lrrr@{}}
\toprule
Model Architecture & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Fit Time\\ (Seconds)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Total\\ Inference Time\\ (Seconds)\end{tabular}} & \multicolumn{1}{c}{F1} \\ \midrule
Random Forest      & 3.69                                                                             & 0.37                                                                                           & 99.8                   \\
\rowcolor{Gray} 
ExtraTrees         & 3.89                                                                             & 0.43                                                                                           & 99.9                   \\
KNeighbors         & 3.90                                                                             & 8.95                                                                                           & 96.0                   \\
\rowcolor{Gray} 
LightGBM           & 5.21                                                                             & 0.15                                                                                           & 99.8                   \\

Catboost           & 9.00                                                                             & 0.38                                                                                           & 99.7                   \\
\rowcolor{Gray} 
Weighted Ensemble  & 46.1                                                                             & 0.45                                                                                           & 99.9                   \\ 

Neural Network     & 85.58                                                                            & 29.9                                                                                           & 99.7                   \\ \bottomrule
\end{tabular}
    \caption{The \name{} representation performs well across models, with training and inference
    times varying depending on the type of modle.}
    \label{fig:app-time}
\end{table}


==> figures/passive/nprint/hard_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
    \centering
    \normalsize
    \resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lrrrrrrrrr@{}}
\toprule
      & \multicolumn{3}{c}{1 Packet}                                                        & \multicolumn{3}{c}{10 Packets}                                                      & \multicolumn{3}{c}{100 Packets}                                                     \\ \cmidrule(l){2-10} 
Model & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{ROC AUC} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{ROC AUC} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{ROC AUC} & \multicolumn{1}{c}{F1} \\ \midrule
MLP   & 0.47                         & 0.88                        & 0.45                   & 0.53                         & 0.90                        & 0.51                   & TBD                          & TBD                         & TBD                    \\
    \rowcolor{Gray} CNN   & Inapplicable                 & Innapplicable               & Innaplicable           & 0.55                         & 0.90                        & 0.53                   & 0.58                         & 0.85                        & 0.56                   \\
RF    & 0.52                         & 0.92                        & 0.50                   & 0.57                         & 0.92                        & 0.55                   & 0.57                         & 0.92                        & 0.55                   \\ \bottomrule
\end{tabular}
    }
    \label{tab:passive-hard}
\end{table}


==> figures/passive/p0f_results.tex <==
\begin{table*}[h]
    \centering
    \small
    % \resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcrrrrrrrrrrrr@{}}
\toprule
                & \multicolumn{1}{l}{}                  & \multicolumn{6}{c}{p0f}                                                                                                                       & \multicolumn{6}{c}{nPrint}                                                                                                                    \\ \midrule
                & \multicolumn{1}{l}{}                  & \multicolumn{2}{c}{1 Packet}                  & \multicolumn{2}{c}{10 Packets}                & \multicolumn{2}{c}{100 Packets}               & \multicolumn{2}{c}{1 Packet}                  & \multicolumn{2}{c}{10 Packets}                & \multicolumn{2}{c}{100 Packets}               \\ \cmidrule(l){3-14} 
Host            & p0f Label                             & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} \\ \midrule
Mac OS          & Mac OS x 10.x                         & 1.00                  & 0.05                  & 1.00                  & 0.28                  & 1.00                  & 0.88                  & 0.99                  & 0.99                  & 1.00                  & 0.99                  & 1.00                  & 0.99                  \\ \midrule
Web Server      & \multirow{6}{*}{Linux 3.11 and newer} & 1.00                  & 0.01                  & 1.00                  & 0.25                  & 1.00                  & 0.74                  & \multirow{6}{*}{0.99} & \multirow{6}{*}{0.99} & \multirow{6}{*}{0.99} & \multirow{6}{*}{1.00} & \multirow{6}{*}{0.99} & \multirow{6}{*}{1.00} \\
Ubuntu 14.4 32B &                                       & 1.00                  & 0.04                  & 1.00                  & 0.20                  & 1.00                  & 0.69                  &                       &                       &                       &                       &                       &                       \\
Ubuntu 14.4 64B &                                       & 1.00                  & 0.04                  & 1.00                  & 0.20                  & 1.00                  & 0.65                  &                       &                       &                       &                       &                       &                       \\
Ubuntu 16.4 32B &                                       & 1.00                  & 0.05                  & 1.00                  & 0.19                  & 1.00                  & 0.68                  &                       &                       &                       &                       &                       &                       \\
Ubuntu 16.4 64B &                                       & 1.00                  & 0.04                  & 1.00                  & 0.24                  & 1.00                  & 0.79                  &                       &                       &                       &                       &                       &                       \\
Ubuntu Server   &                                       & 1.00                  & 0.05                  & 1.00                  & 0.25                  & 1.00                  & 0.74                  &                       &                       &                       &                       &                       &                       \\ \midrule
Windows 10      & \multirow{5}{*}{Windows 7 or 8}       & 0.99                  & 0.00                  & 0.98                  & 0.02                  & 0.98                  & 0.09                  & \multirow{5}{*}{1.00} & \multirow{5}{*}{1.00} & \multirow{5}{*}{1.00} & \multirow{5}{*}{1.00} & \multirow{5}{*}{1.00} & \multirow{5}{*}{1.00} \\
Windows 10 Pro  &                                       & 0.99                  & 0.01                  & 0.98                  & 0.04                  & 1.00                  & 0.14                  &                       &                       &                       &                       &                       &                       \\
Windows 7 Pro   &                                       & 1.00                  & 0.04                  & 1.00                  & 0.23                  & 1.00                  & 0.71                  &                       &                       &                       &                       &                       &                       \\
Windows 8.1     &                                       & 0.99                  & 0.05                  & 0.99                  & 0.25                  & 0.99                  & 0.77                  &                       &                       &                       &                       &                       &                       \\
Windows Vista   &                                       & 1.00                  & 0.01                  & 1.00                  & 0.27                  & 1.00                  & 0.71                  &                       &                       &                       &                       &                       &                       \\ \midrule
Kali Linux      & No output                             & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} \\ \bottomrule
\end{tabular}
%   }%
    \caption{
        Performance of \name{}ML vs. p0f for passive
        OS fingerprinting. \name{}ML is capable of finer granularity for OS
        fingerprinting and achieves near perfect precision and recall when
        compared directly to p0f. While p0f never provides any OS estimate for
        Kali Linux, we include it for testing fine-grained OS classification with
        \name{}ML.
    }
    \label{tab:p0f}
\end{table*}


==> figures/performance/mem.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
    \centering
    \normalsize
    \resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lrrr@{}}
\toprule
Problem                      & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}PCAP \\ (Headers Only)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Uncompressed \\ nPrint\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Compressed \\ nPrint\end{tabular}} \\ \midrule
Passive OS Detection         & Todo MB                                                                            & 3 GB                                                                               & 64 MB                                                                            \\
    \rowcolor{Gray} Application Identification   & 1.7 MB                                                                             & 61 MB                                                                              & 1.6 MB                                                                           \\
Active Device Fingerprinting & 18 MB                                                                              & 716 MB                                                                             & 15 MB                                                                            \\ \bottomrule
\end{tabular}
    }
    \caption{\name{} compresses efficiently on disk due to its binary format.}
    \label{tab:compress}
\end{table}


==> figures/performance/model-time.tex <==
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[h]
    \centering
    \normalsize
    \resizebox{\columnwidth}{!}{%
\begin{tabular}{lrrr}
\hline
                             & \multicolumn{3}{c}{Training Time (Seconds)}                                                                                                                                                     \\ \cline{2-4} 
\multicolumn{1}{c}{Problem}  & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}MLP\\ (50 Epochs)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}CNN\\ (50 Epochs)\end{tabular}} & \multicolumn{1}{c}{RF} \\ \hline
Passive OS Detection         & 3.5                                                                           & 8.5                                                                           & 6                      \\
\rowcolor{Gray} 
Active Device Fingerprinting & 3.5                                                                           & 6.5                                                                           & 1                      \\
Application Identification   & 1                                                                             & 3                                                                             & .5                     \\ \hline
\end{tabular}
    } %
    \caption{Models train quickly on \name{}'s standard representation.}
    \label{tab:perf-model}
\end{table}


==> figures/performance/nprint.tex <==
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
    \centering
    \normalsize
    \resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lrrr@{}}
\toprule
\multicolumn{1}{c}{Problem}  & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Unique LOC\\ (Python)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Input\\ (Packets)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}nPrint\\ (Seconds)\end{tabular}} \\ \midrule
Passive OS Detection         & 27                                                                                & 1,343,920                                                                     & 49                                                                             \\
\rowcolor{Gray} 
Active Device Fingerprinting & 16                                                                                & 274,010                                                                       & 13                                                                             \\
Application Identification   & 33                                                                                & 48,816                                                                        & 12                                                                             \\ \bottomrule
\end{tabular}
    } %
    \caption{nPrint transforms packets quickly.}
    \label{tab:perf-nprint}
\end{table}


==> figures/performance/perf.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
    \centering
    \normalsize
    \resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lrrr@{}}
\toprule
Problem                    & \# Packets &
    \begin{tabular}[c]{@{}c@{}}nPrint Transformation \\ (Seconds) \end{tabular} & \begin{tabular}[c]{@{}c@{}} LOC \\ (Python)\end{tabular} \\ \midrule
Active Fingerprinting      & 274,010           & 14 & 16                                                                       \\
\rowcolor{Gray} 
Passive OS Detection       & 1,343,920         & 49 & 27                                                                       \\
Application Identification & 46,816            & 12                                          & 33                                                                       \\ \bottomrule
\end{tabular}
     } %
    \caption{\name{} currently transforms over 1 million packets per minute on a
    single thread.}
    \label{tab:perf}
\end{table}


==> figures/performance/pipeline.tex <==
\begin{table*}[h]
    \normalsize
    \centering
\begin{tabular}{@{}lr|r|r|rrr|@{}}
\toprule
                             & \multicolumn{1}{c|}{}                                                              & \multicolumn{1}{c|}{Input}      & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Packet \\ Transformation\end{tabular}} & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Model \\ Training\end{tabular}}                                                                                                          \\ \cmidrule(l){3-7} 
\multicolumn{1}{c}{Problem}  & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Unique LOC\\ (Python)\end{tabular}} & \multicolumn{1}{c|}{\# Packets} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}nPrint\\ (Seconds)\end{tabular}}       & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}FFN\\ (50 Epochs)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}CNN\\ (50 Epcohs)\end{tabular}} & \multicolumn{1}{c|}{RF} \\ \midrule
Passive OS Detection         & 27                                                                                 & 1,343,920                       & 49                                                                                    & 3.5                                                                           & 8.5                                                                           & 1                       \\
\rowcolor{Gray} 
Active Device Fingerprinting & 16                                                                                 & 274,010                         & 13                                                                                    & 3.5                                                                           & 6.5                                                                           & 6                       \\
Application Identification   & 33                                                                                 & 48,816                          & 12                                                                                    & 1                                                                             & 3                                                                             & .5                      \\ \bottomrule
\end{tabular}
    \caption{\name{} allows for rapid testing of traffic analysis problems,
    requiring as few as 16 lines of code to adapt to entirely new contexts.
    Furthermore, each models type trains quickly on the \name{} representation.}
    \label{tab:perf}
\end{table*}


==> figures/performance/rate.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
    \centering
    \normalsize
\begin{tabular}{@{}rrr@{}}
\toprule
PPS (million)                     & \multicolumn{1}{l}{Avg Throughput} & \multicolumn{1}{l}{Packet Loss \%} \\ \midrule
0.5         & 1.3~Gbps                             & 0.11
\\ \rowcolor{Gray}
1 & 2.6~Gbps                           & 0.35                          \\
1.5   & 4~Gbps                           & 0.44                         \\ \bottomrule
\end{tabular}
    \caption{Single threaded \name{} live traffic processing performance.}
    \label{tab:linerate}
\end{table}


==> sections/active.tex <==
\subsection{Active Device Fingerprinting}
\label{sec:active}

First, we examine the utility of \name{}ML to extract features from packets in the
context of active device fingerprinting. We compare the
performance of models trained on the \name{} representation to Nmap, perhaps the most popular
device fingerprinting tool, which has been developed for over 20 years.

\paragraph{Input (Packets).}

We use a dataset of labeled devices and fingerprints to compare \name{}ML's
performance to Nmap's hand-engineered features. Holland \etal{} previously used
a subset of Nmap's probes to fingerprint network device vendors at
Internet scale~\cite{holland2020classifying}. They curate a labeled dataset of
network devices through an iterative clustering technique on SSH, Telnet, and
SNMP banners, which provides a list of labeled network devices to Nmap.

Although this previous work was concerned with fingerprinting devices at scale, we
are concerned with \name{}ML's classification performance against Nmap's full suite of
features. As such, we downsample the labeled network device dataset to create a
set of devices to compare the classification performance of \name{}ML with Nmap. We further
expand the types of devices we are testing to test the adaptability of \name{}ML
across a larger range of device types. To this end, we add a new device category
to the dataset: Internet of Things (IoT) devices. We gather labels for four
types of IoT devices, two IoT cameras and two IoT TV streaming devices through
Shodan~\cite{shodan}. Table~\ref{tab:nmap-heuristic} shows the final dataset.

Holland~\etal{}'s dataset includes the Nmap output and raw packet responses for
each label in the dataset. We modify Nmap to output the raw responses for each
probe and Nmap each IoT device added through Shodan labeling. We only have access to the \textit{responses} to the probes that Nmap sends, not
the actual sent probes, as we cannot re-scan the labeled router dataset
due to the chance that the device underneath the IP address may have changed.

\input{figures/active/nmap-heuristic.tex}

\paragraph{Packet Transformation and Data Representation.}
\label{subsec:active-transform}
Nmap transforms the responses to each probe into a fingerprint using a series of
varyingly complex tests developed for decades. Table~\ref{tab:nmap-tests} in
Appendix~\ref{appendix-nmap} outlines the full set of
tests Nmap performs on the probe responses, which includes complex features computed
across sets of packets. We use this fingerprint for our
evaluation in two ways. First, Nmap compares the fingerprint generated to its
database, making a classification of the remote device. Second, we take the
fingerprint and encode each test as a categorical feature, creating a feature
vector to be used with machine learning methods. Holland \etal{} show that this technique 
is effective using Nmap's closed-port probes, which comprise only 6 of the 16
probes Nmap sends to each device. We consider \textit{every} test Nmap conducts 
when transforming each fingerprint into a feature vector. 

\name{}ML uses the raw responses generated from the modified version of Nmap to build a
\name{} for each device. \name{}ML uses the same response packets that Nmap uses to
build each \name{}. Further, while Nmap computes many of its features across both
sent and received packets, we only have access to the received packets in each
\name{}.

We configure \name{}ML to include IPv4, TCP, and ICMP headers in each \name{},
resulting in 1,024 features for each individual packet. Here we note that while configuring \name{} and
\name{}ML requires some user intervention, namely indicating the type of traffic to include in the output via a command-line flag, this configuration 
requires significantly less work when compared with manually defining, extracting, and representing features from multiple traffic protocols.
\name{}ML aggregates all responses from each device to create a 21-packet \name{} for each device. We
point out that there are 21 packets 
in each \name{}, while Nmap sends only 16 probes to the device. Nmap re-sends
probes that do not garner a response up to three times. It uniquely re-names
these probes. Rather than disambiguate the names, which is unreliable due to the
unique naming scheme, we consider each uniquely named Nmap response as a packet in
the \name{}. This does not give us access to any information that Nmap does not
use, and at worst duplicates data already in the \name{}. \name{}ML fills any
probe response with -1s if the device did not respond to the probe. Finally, as each
probe is specifically named, we sort each aggregated \name{} created by
\name{}ML by the probe name to ensure consistent order across all samples.

\input{figures/active/nprint-vs-nmap.tex}
\input{figures/active/nmap-eval.tex}

\paragraph{Nmap's heuristics perform poorly for some devices.}
Nmap compares its generated fingerprint to a hand-curated fingerprint database
using a carefully-tuned heuristic. Table~\ref{tab:nmap-tests} in
Appendix~\ref{appendix-nmap} shows weights of this heuristic. Nmap either outputs a direct guess of the device,
which it is more confident in, or an aggressive guess, where there is less
confidence in the output. Table~\ref{tab:nmap-heuristic} shows the performance
of this heuristic on the entire dataset using both direct and aggressive
metrics. We see that Nmap's performance is low across the entire dataset with
the exception of Cisco, Juniper, and Adtran devices, for which it has high
precision with relatively low recall. We notice a trend in the devices that Nmap
is accurate at classifying: older, North American based routers. Of all of the
IoT devices in the dataset, Nmap's highest heuristic precision is .01.



%\begin{figure}[t]
%  \centering
%  \begin{subfigure}[b]{0.85\columnwidth}
%    \centering
%      \includegraphics[width=\columnwidth]{figures/active/nmap/pr.pdf}
%    \label{fig:active-pr-nm}
%    \caption{Nmap PR}
%  \end{subfigure}
%  \begin{subfigure}[b]{0.85\columnwidth}
%    \centering
%    \includegraphics[width=\columnwidth]{figures/active/nprint/pr.pdf}
%    \label{fig:active-pr}
%      \caption{\name{}ML PR}
%  \end{subfigure}
%    \caption{\name{}ML achieves higher performance than expert-derived features,
%    even without access to Nmap's sent probes.}
%  \label{fig:active-compare-nprint}
%\end{figure}

\input{figures/active/time.tex}
\begin{figure}[t]
  \centering
    \centering
    \begin{subfigure}[b]{0.8\linewidth}
      \centering
      \includegraphics[width=\linewidth,trim={0 85 0 60},clip]{figures/active/heatmaps/ipv4_v2.pdf}
      \caption{IPv4}
      \label{fig:active-ipv4-heat}
    \end{subfigure}
    \begin{subfigure}[b]{0.8\linewidth}
      \centering
      \includegraphics[width=\linewidth,trim={0 85 0 85},clip]{figures/active/heatmaps/tcp_v2.pdf}
      \caption{TCP}
      \label{fig:active-tcp-heat}
    \end{subfigure}
    \begin{subfigure}[b]{0.8\linewidth}
      \centering
      \includegraphics[width=\linewidth,trim={0 165 0 165},clip]{figures/active/heatmaps/icmp_v2.pdf}
      \caption{ICMP}
      \label{fig:active-icmp-heat}
    \end{subfigure}
    \caption{
        Per-bit feature importance for active fingerprinting, computed by
        summing the feature importance for each individual \name{} in the 21 packet \name{}
        created for each device. Brighter colors are more important. Given the \name{} representation,
        ML models can learn important features (e.g., IP TTL, window size), as opposed to
        relying on manual engineering.
    }
    \label{fig:active-heat}
\end{figure}

\input{figures/passive/p0f_results.tex}

\paragraph{\name{}ML outperforms an AutoML-enhanced Nmap.}
To directly compare Nmap's long-developed techniques for extracting differentiating features from
network protocols to \name{}ML, we enhance
Nmap by replacing its heuristic with AutoML. We take each one-hot-encoded Nmap
fingerprint and run the AutoML pipeline, creating optimized models for the extracted
features. We also run \name{}ML on the \name{} representation 
generated for each device.



Table~\ref{tab:nprintvsnmap} shows the average precision score, used to summarize a precision-recall curve, 
of the highest performing classifier for Nmap and \name{}ML~\cite{sklearn:aps}. Immediately, we see that not only
can models trained on the \name{} representation differentiate the devices without manual feature
engineering, \name{}ML outperforms Nmap's hand-engineered features.
Table~\ref{tab:nmap-perf} examines the best performing model for both
Nmap and \name{}ML. We see that \name{}ML outperforms Nmap's long-developed features
in every metric without access to the sent probes. 



Table~\ref{tab:active-time} examines the training and inference time of the two
highest performing models for both Nmap and \name{}ML. We see that although the
highest performing \name{}ML model takes longer to train than on Nmap's
features, models trained on the \name{} representation can achieve higher F1
scores than models trained on Nmap's features with a lower training time and
faster inference speed. Figure~\ref{fig:active-heat} shows a heatmap of the
feature importance gathered from the random forest model trained with \name{}ML.
We find that the TCP source port of the response probes are one of the more
important features in classifying the device vendor. Upon further inspection, we
find that Nmap does a port scan to find an open port to sent its open-port
probes to. The IoT devices each have a specific port that is found to be open
during the port scan that identify the class of devices from the routers. We
also see that the IP TTL and TCP window size are helpful in identifying the
device.







==> sections/app.tex <==
\subsection{DTLS Application Identification}
\label{sec:app}

We test the ability of \name{}ML to identify a set of applications
through their DTLS handshakes. We aim to automatically identify the application
and browser that generated a DTLS handshake with \name{}ML when provided with the
handshake traffic. MacMillan \etal{} examined the feasibility of fingerprinting
Snowflake, a pluggable transport for Tor that uses WebRTC to establish
browser-to-browser connections~\cite{macmillan2020evaluating}, which is built to
be indistinguishable from other WebRTC services. They collect almost 7,000 DTLS
handshakes from four different services: Facebook Messenger, Discord, Google
Hangouts, and Snowflake, across two browsers: Firefox and Chrome. They then write a protocol parser and 
extract and engineer semantic features from the handshakes to show that Snowflake is identifiable with
perfect accuracy. 

We are interested demonstrating \name{}ML's ability to automate this process
entirely. This DTLS classification problem highlights both \name{}ML's ability to
adapt to entirely new tasks that involve packet payloads, and \name{}ML's performance in a noisy environment, as
the packet traces vary in length due to retransmission in the UDP-based
handshakes.
 
\input{figures/app/dataset.tex}

\paragraph{Input (Packets).}
Table~\ref{tab:app-dataset} shows an overview of the nearly 7,000 DTLS
handshakes in the dataset. While MacMillan \etal{} examine the classification
task solely at the application level, we \textit{further} split the
classification task into the specific (browser, application) pair created the
handshake, increasing the number of classes in the task from four to seven.
Snowflake traffic is specific to the Firefox browser and did not contain any Chrome
instances.




\paragraph{Packet Transformation and Data Representation.}
We configure \name{}ML to transform each handshake, which was captured and
filtered as a PCAP file, into a \name{}. We vary the configuration of \name{}ML
to test \name{}ML
under a variety of constraints. Table~\ref{tab:case-studies} shows these
configurations. The number of packets in the packet captures varies from 4 to 43 due
to both client behavior and packet retransmissions. \name{}ML pads each
fingerprint to the maximum capture size with -1s and allows the models trained
on the \name{} representation to identify important features in noisy traffic.

\paragraph{\name{}ML can automatically detect features in a noisy environment.}
We run \name{}ML on the handshakes in \name{} format. The weighted ensemble
classifier trained on the \name{} representation achieves a perfect ROC AUC score, 99.8\% accuracy,
and 99.8\% F1 score. \name{}ML can almost perfectly identify the
(browser, application) pair that generates each handshake. While in prior work
manually engineered features achieved the same accuracy on an easier
version of the problem, \name{}ML avoids model selection and feature engineering 
entirely, matching the performance of manual features and
models on a more difficult instance of the
problem~\cite{macmillan2020evaluating}. Finally, we examine models trained on
the 
\name{} representation using different combinations of headers in each packet in the traffic.
Table~\ref{tab:case-studies} shows that models trained on the \name{}
representation can perform
this task with high accuracy using \textit{only} the UDP headers in each packet.

\input{figures/app/time.tex}

\paragraph{\name{}ML performs well across models and trains quickly.}
Table~\ref{fig:app-time} shows the F1 score, training time, and total inference
time on the testing dataset for each non-ensemble classifier trained and the
weighted ensemble classifier with the highest overall performance. The \name{}
representation works across models, with inference and training time varying. \name{} 
working well across different models is important as some environments require
different optimizations. For example, classification in streaming environments
may prefer faster inference time over the highest performing model.

\begin{figure}[t]
  \centering
    \begin{subfigure}[b]{0.8\linewidth}
      \centering
      \includegraphics[width=\linewidth,trim={0 85 0 60},clip]{figures/app/heatmaps/ipv4_v2.pdf}
      \caption{IPv4}
      \label{fig:app-ipv4-heat}
    \end{subfigure}
    \begin{subfigure}[b]{0.8\linewidth}
      \centering
      \includegraphics[width=\linewidth,trim={0 165 0 165},clip]{figures/app/heatmaps/udp_v2.pdf}
      \caption{UDP}
      \label{fig:app-udp-heat}
    \end{subfigure}
    \begin{subfigure}[b]{0.8\linewidth}
      \centering
      \includegraphics[width=\linewidth,trim={0 165 0 165},clip]{figures/app/heatmaps/payload_v2.pdf}
      \caption{DTLS}
      \label{fig:app-payload-heat}
    \end{subfigure}
    \caption{
        Per-bit feature importance for (browser, application) identification,
        computed by summing the feature importance for each individual \name{}
        in the 43 packet \name{} created for each handshake. 
        Brighter colors are more important. Given the \name{} representation,
        ML models can automatically learn important features (e.g., length), as opposed to
        relying on manual engineering.
    }
    \label{fig:app-heat}
\end{figure}

\paragraph{\name{}ML can be used to understand semantic feature importance.}
We use \name{}ML to map feature importance to their semantic meaning.
Figure~\ref{fig:app-heat} shows a heatmap of the feature importance gathered
from the highest performing random forest model trained on the \name{}
representation. In this instance, the successive lengths of the headers (steps in the
handshake) and the information in the DTLS payload drive much of the performance in \name{}ML. 


==> sections/case_studies.tex <==
\section{Case Studies}
\label{sec:case-studies}

In this section, we highlight the versatility and performance of \name{}. Table
~\ref{tab:case-studies} presents the breadth of problems that \name{}ML can be
leveraged for, summarizing eight case studies tested with \name{}ML. This
section examines those case studies in more depth: We show that \name{}ML
can match or beat the performance of existing bespoke approaches for each of
these problems.

\input{active}
\input{passive}
\input{app}
\input{extra_cs}


==> sections/extra_cs.tex <==
\subsection{Additional Case Studies}
\label{sec:netml}

In this section, we apply \name{}ML across several additional case studies, as
summarized in
Table~\ref{tab:case-studies}.
For brevity, we describe each study and show the \name{}ML command associated with the performance results shown in the table.
In each case study we ran \name{}ML with a range of packet counts. We include the best performing commands here.

\subsubsection{netML Challenge Examples}
\label{subsec:netml}

We study the breadth of \name{} and \name{}ML in context of the
netML challenge, a public traffic analysis challenge that consists of three flow-level traffic analysis problems: malware detection for IoT devices, 
intrusion detection, and traffic identification\cite{barut2020netml}. Each task is further divided into easier and harder versions of the task by changing the
granularity of the labels, increasing or decreasing the number of classes to be identified. The creators released a set of hand-engineered features for each
problem, equating to a semantic representation of each flow. Participants are invited to 
train and tune any type of model with the goal of achieving the highest performance for each task. 

We aim to see if \name{}ML can outperform the hand-engineered features and hand-tuned models published on the netML 
leaderboard~\cite{netmlleaderboard}. Unfortunately, the authors only released the features for each traffic flow in the dataset,
not the raw traffic data. As such, we faithfully recreated the raw datasets with help from the original authors. In the vast majority
of cases, we exactly match the number of samples for each class in each task. However, due to this recreation effort we do not necessarily have the same training and
testing split as the original challenge dataset, and as such our results do not reflect a perfect comparison. Finally, we remove the IP addresses from each packet in our sample when running \name{}ML to match the original challenge.

Table~\ref{tab:case-studies} shows the results for each of the three netML
challenge case studies. In every task but one \name{}ML outperforms the highest
performing hand-tuned model on the netML leaderboard~\cite{netmlleaderboard} without manual feature engineering. 
Below we show the \name{}ML commands used to create the full traffic analysis pipeline for each task.


\begin{lstlisting}
# Intrusion Detection
$ nprintml -L labels.txt -a pcap \
--pcap-dir traffic_flows/        \
-4 -t -u -c 5                    \
-x "ipv4_src.*|ipv4_dst.*" 
\end{lstlisting}

\vspace{.5cm}
\begin{lstlisting}
# Malware Detection
$ nprintml -L labels.txt -a pcap \ 
--pcap-dir traffic_flows/        \ 
-4 -t -u -c 10                   \
-x "ipv4_src.*|ipv4_dst.*"
\end{lstlisting}

\begin{lstlisting}
# Traffic Identification (No Payload bytes)
$ nprintml -L labels.txt -a pcap \
--pcap-dir traffic_flows/        \
-4 -t -u -c 5                    \
-x "ipv4_src.*|ipv4_dst.*"
\end{lstlisting}

\begin{lstlisting}
# Traffic Identification (10 Payload bytes)
$ nprintml -L labels.txt -a pcap \
--pcap-dir traffic_flows/        \
-4 -t -u -p 10 -c 5              \
-x "ipv4_src.*|ipv4_dst.*" 
\end{lstlisting}

\subsubsection{Mobile Country of Origin}
\label{subsec:mobile}

We examine the ability of \name{}ML to determine the country of origin of mobile application traces using the Cross Platform dataset~\cite{crossmarketdataset}.
Specifically, we use \name{}ML to train a model that can determine if the mobile application trace originated in China, the United States, or India.
Table~\ref{tab:case-studies} shows the performance of the best model trained on the task. Ultimately, \name{}ML can perform this task with over 96\% accuracy
using the IPv4, TCP, and UDP headers of each packet. The \name{}ML command to create the traffic analysis pipeline is shown
below.

\begin{lstlisting}
$ nprintml -L labels.txt -a pcap \ 
--pcap-dir application_traces/   \
-4 -t -u -p 50 -c 25             \
-x "ipv4_src.*|ipv4_dst.*"
\end{lstlisting}

\subsubsection{Streaming Video Providers}
\label{subsec:video}

Last, we demonstrate how \name{} and \name{}ML can enable rapid hypothesis
testing for traffic analysis. Bronzino~\etal{} examined the feasibility of
training a model to infer the streaming video quality of different video
services (Netflix, YouTube, Amazon, and Twitch)~\cite{bronzino2019inferring}.
Rather than video quality, we wish to train a model that can differentiate the
video services. Our hypothesis is that each streaming video service player may
exhibit individualistic flow behavior to deliver video traffic, which may then
enable the identification of each service. We filter each individual video
traffic trace for only SYN packets (to capture flow creation) and create a full
traffic analysis pipeline using the command below. As shown in
Table~\ref{tab:case-studies}, the highest performing model trained on \name{}
can identify the streaming service with 98\% accuracy.

\begin{lstlisting}
$ nprintml -L labels.txt -a pcap \
--pcap-dir video_traces          \
-4 -t -u -R -c 25                \
-f "tcp[13] == 2"               
\end{lstlisting}


==> sections/passive.tex <==
\subsection{Passive OS Fingerprinting}\label{sec:passive}

We study \name{} in the context of passive OS fingerprinting: determining
the operating system of a device from network traffic. We compare
the performance of \name{}ML to p0f,
one of the most well-known and commonly used passive OS fingerprinting tools.
Ultimately, we find that \name{}ML can perform OS detection with much higher
recall rate than p0f, using much smaller packet sequences. Further, we find that
\name{}ML can uncover fine-grained differences in OSes. We 
highlight that \name{}ML is able to be used in a variety of manners including
single-packet OS detection and using sequences of packets.

p0f uses an array of traffic fingerprinting mechanisms to identify the OS
behind any TCP/IP communication. p0f relies on a user-curated database of
signatures to determine the operating system of any given device. p0f generates semantic 
fingerprints from device traffic and looks for direct matches in its database in
order to identify the OS. We note that p0f's fingerprinting capabilities
include \textit{much} more breath than is considered in this case study, as it
contains signatures for not only OS detection, but browser identification,
search robots, and some commonly used applications. We
specifically aim to test if models trained on the \name{} representation can exceed the performance
of p0f on a common task for the tool and test if \name{}ML can be used for
automated, fine-grained OS detection.

\paragraph{Input (Packets).}
We use the CICIDS2017 intrusion detection evaluation dataset, which
contains PCAPs of over 50~GB of network traffic over the course of 5
days~\cite{sharafaldin2018toward}. The traffic contains labeled operating
systems ranging from Ubuntu to Windows to MacOS. There are 17 hosts in the IDS
dataset, but we find only 13 with usable traffic. The usable devices are seen in
the first column of Table~\ref{tab:p0f}.

\paragraph{Packet Transformation and Data Representation.}
We vary the amount of traffic available to p0f and \name{}ML to compare
performance in different settings. We use the first 100,000 packets seen for
each device and split them into sets of 1, 10, and 100 packet samples (\ie,
100,000 1-packet PCAPs, 10,000 10 packet PCAPS, etc.) to be used with both. This
results in three separate classification problems, each problem using the same
traffic, but varying amounts of information the classification technique 
accesses in each sample.

p0f extracts several fields from each packet and compares extracted values
against a fingerprint database to find a matching OS for the extracted fields.
We run p0f, without modifications, on each of the 1, 10, and 100 packet samples
created from each device's traffic. We create separate \name{}ML pipelines for
the 1, 10, and 100 packet traffic samples, configuring it to remove the IP source address, IP destination address, IP
identification, TCP source and destination ports, and TCP sequence and acknowledgement numbers from each
\name{} to avoid learning direct identifiers of specific devices rather than
general operating system characteristics. Further, we configure \name{}ML to only
use IP and TCP headers to fairly compare \name{}ML with p0f.

p0f outputs an operating system guess only on packets that directly
match a fingerprint in p0f's database, so the number of estimates varies between
samples. We treat each estimate as a vote. For each sample, we tally the number
of correct votes, incorrect votes, and cases where p0f offered no estimate.
Using these values we calculate the precision and recall for each experiment.
Table~\ref{tab:p0f} shows the precision and recall for each separate experiment.

Table~\ref{tab:p0f} illustrates the relatively coarse-grained output generated
by p0f. For example, p0f classifies all Ubuntu devices, and the web server, as
``Linux 3.11 and newer'', and all of the Windows devices as ``Windows 7 or 8''.
Table~\ref{tab:p0f} shows that p0f generally increases in performance when given
access to more packets in a sample, and that it is precise when it does
make an estimate. Unfortunately, p0f's recall is generally
quite low until given access to 100 packet samples for a device, as p0f does not
offer any estimates for many samples. Finally, p0f never outputs a
single vote for the Kali Linux traffic samples.

\begin{figure}[t]
  \centering
  \begin{minipage}[t]{\columnwidth}
    \centering
    \begin{subfigure}[b]{0.8\linewidth}
      \centering
      \includegraphics[width=\linewidth,trim={0 85 0 60},clip]{figures/passive/heatmaps/ipv4_v2.pdf}
      \caption{IPv4}
      \label{fig:passive-ipv4-heat}
    \end{subfigure}
    \begin{subfigure}[b]{0.8\linewidth}
      \centering
      \includegraphics[width=\linewidth,trim={0 85 0 85},clip]{figures/passive/heatmaps/tcp_v2.pdf}
      \caption{TCP}
      \label{fig:passive-tcp-heat}
    \end{subfigure}
    \caption{
        Per-bit feature importance for passive OS detection.
        Brighter colors are more important. Given the \name{} representation,
        ML models can automatically discover important features (e.g. IP TTL,
        window size), as opposed to
        relying on manual engineering.
}
    \label{fig:passive-heat}
  \end{minipage}
\end{figure}

\paragraph{\name{}ML can perform OS classification with high recall and few 
packets.} 
To directly compare \name{}ML to p0f, we use the ``p0f Label'' in
Table~\ref{tab:p0f} as a label for each
host and train each classifier using the 3 coarse-grained classes on the same
samples that p0f was executed on. Table~\ref{tab:p0f} shows the results of this
classification. As shown, models trained on the \name{} representation
achieve nearly the same precision as p0f while drastically improving upon p0f's
recall. Interestingly, with only one packet, a model
trained on the \name{} representation can outperform p0f when given access to 100 packet
samples. We also see very slight improvements in model performance when
increasing the number of packets in each \name{}. Figure~\ref{fig:passive-heat} shows a heatmap of the feature importance
gathered from the highest performing random forest model trained with \name{}ML. For the IPv4 header, 
the most important features are in the time-to-live (TTL)
field and, to a lesser degree, the IPID field. These results confirm past
observations that TTL IPID can be used for OS detection, because different
operating systems use different default values for those
fields~\cite{10.1145/637201.637243, ttl}.
In the TCP header, the window size field is the most important feature. We also
observe that certain bits in the TCP options can help determine OS as some OSes
include particular options by default such as maximum segment size, window
scaling, or selective acknowledgement permitted. 

\begin{figure}[t]
  \centering
  \begin{subfigure}[b]{0.89\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/passive/automl/pr.png}
    \caption{\name{}ML PR.}
    \label{fig:passive-pr}
  \end{subfigure}
  \begin{subfigure}[b]{0.9\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/passive/automl/cfmx.png}
    \caption{\name{}ML Confusion Matrix.}
    \label{fig:passive-cfmx}
  \end{subfigure}
  \caption{Passive OS fingerprinting PR and confusion matrix for \name{}ML.
    Models trained on the \name{} representation learn to identify operating
    systems at a finer granularity (\eg, versions) than p0f.}
  \label{fig:passive-compare}
\end{figure}

\paragraph{\name{}ML can reveal fine-grained differences in OSes.}
Next, we aim to discover if models trained on the \name{} representation can enable automated passive OS
detection at a more fine-grained level. We take the same 100-packet
samples and train each model using the ``Host'' column of Table~\ref{tab:p0f} as
a label for each sample, resulting in a 13-class classification problem. 
Figure~\ref{fig:passive-pr} shows the PR curve of the highest performing model.

Figure~\ref{fig:passive-cfmx} examines the performance of the
model trained on the \name{} representation in more detail. The classifier separates
operating system characteristics, with almost all of the confusion being
\textit{within the same operating system}. The
classifier can separate the devices into more fine-grained classes than
p0f's original output, finding differences in Windows Vista and Kali Linux that
are not encoded into p0f. Figure~\ref{fig:passive-cfmx} also
illustrates a challenge in fine-grained OS detection, as bit version differences
of the same OS tend to lead to confusion. This result is unsurprising, as we
anticipate the network stack for an OS would be similar between different bit
versions.

\paragraph{\name{}ML differentiates OSes, not simply devices.}
We seek to verify that \name{}ML detects operating systems generally,
rather than learning to identify specific devices on the network. We construct an experiment
where we compare sets of devices that share a common OS. We take the five Ubuntu
hosts and five Windows hosts in the dataset and set up a binary classification
task where we iteratively select pairs from the two lists to train a model,
and test against the remaining hosts in the lists. 

\name{}ML differentiates between Ubuntu and Windows machines with perfect balanced
accuracy, ROC AUC scores, and F1 scores no matter which device pair was used for
training. This is due to the different initial IP time-to-live that is set by
the two operating systems which the model immediately learns. This experiment
illustrates that models can successfully identify operating systems
generally from the \name{} representation, as opposed to memorizing individual device characteristics.

Finally, we ensure that \name{} is not memorizing the \textit{locations} of the
hosts in a network via the TTL of the devices\footnote{Note that p0f does use
location along the path as a feature. p0f attempts to guess the initial TTL by
assuming that the value is one of 64, 128, or 255. Decremented TTLs are then
used to calculate ``distance'' (\eg, location on the path) from the initial
TTL.}. In this experiment, we seek to limit \name{} to initial TTLs. The CICIDS2017
traffic was captured on end hosts. Given this, we filter and split the PCAPs to only include packets whose source was also the capture host. This ensures that \name{} only has access to the initial TTL values for each host rather than a decremented value that may indicate the location of the device. Figure~\ref{fig:passive-ittl-cfmx} shows the results of the experiment  
using 10-packet samples. We see that the confusion of \name{} still lies
\textit{within individual operating systems}. \name{} still differentiates the
Web Server and Windows Vista from the other classes. Kali Linux is omitted from
this experiment as it was not found to initiate any traffic flows in the traffic
examined.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/passive/ttl-test/cfmx.png}
    \caption{\name{}ML Confusion Matrix using only initial TTL values.}
    \label{fig:passive-ittl-cfmx}
\end{figure}

